Redefining DDoS Attack Detection Using A Dual-Space Prototypical Network-Based Approach

Distributed Denial of Service (DDoS) attacks pose an increasingly substantial cybersecurity threat to organizations across the globe. In this paper, we introduce a new deep learning-based technique for detecting DDoS attacks, a paramount cybersecurity challenge with evolving complexity and scale. Specifically, we propose a new dual-space prototypical network that leverages a unique dual-space loss function to enhance detection accuracy for various attack patterns through geometric and angular similarity measures. This approach capitalizes on the strengths of representation learning within the latent space (a lower-dimensional representation of data that captures complex patterns for machine learning analysis), improving the model's adaptability and sensitivity towards varying DDoS attack vectors. Our comprehensive evaluation spans multiple training environments, including offline training, simulated online training, and prototypical network scenarios, to validate the model's robustness under diverse data abundance and scarcity conditions. The Multilayer Perceptron (MLP) with Attention, trained with our dual-space prototypical design over a reduced training set, achieves an average accuracy of 94.85% and an F1-Score of 94.71% across our tests, showcasing its effectiveness in dynamic and constrained real-world scenarios.

==> discussions.tex <==
\section{Contributions}

The detection of Zero-Day DoS attacks within the project hinges on several innovative strategies and mechanisms that specifically target the unknown and unpredictable characteristics of such attacks. Here's a breakdown of how the detection process is approached:

Multi-Modality Data Utilization
The model leverages multi-modality data, including network traffic, server logs, system events, and user activities, to create a comprehensive dataset that is instrumental in identifying patterns indicative of Zero-Day DoS attacks. This broad spectrum of data sources enriches the model's input, providing a holistic view of network behavior and anomalies that could signify a Zero-Day attack.

Adaptive Learning Mechanisms
Adaptive learning mechanisms enable the model to adjust to new and evolving attack patterns dynamically. This flexibility is crucial for detecting Zero-Day attacks, which exploit previously unknown vulnerabilities. By continuously learning from new data, the model can identify unusual patterns that deviate from known attack signatures, thus targeting the inherent unpredictability of Zero-Day threats.

Transfer Learning Techniques
The project employs transfer learning to enhance the model's ability to recognize Zero-Day DoS attacks. By transferring knowledge from models trained on similar tasks, the framework reduces the need for extensive new data on the specific Zero-Day vulnerability being exploited. This method is particularly valuable for Zero-Day attack detection, where the novelty of the attack means limited specific data is available for training.

Attention Mechanisms
The incorporation of attention mechanisms allows the model to focus on the most salient features within the data, which are critical for distinguishing between normal activity and potential Zero-Day DoS attacks. This focus on relevant data points helps in identifying subtle anomalies that characterize the unknown nature of Zero-Day vulnerabilities.

Prototypical Networks and Few-Shot Learning
Prototypical Networks, as part of a few-shot learning strategy, enable the model to generalize from limited examples. This capability is essential for Zero-Day DoS attack detection, where the model must accurately identify attacks with minimal prior data. By learning class prototypes and minimizing the distance between query sample embeddings and their corresponding class prototypes, the model can effectively detect novel attack patterns.

Continuous Online Learning
The framework's online learning component ensures real-time adaptability by continuously updating the model with incoming data. This ongoing adaptation is key to maintaining detection efficacy against the rapidly evolving landscape of Zero-Day DoS attacks.

Novel Evaluation Metric
A novel evaluation metric assesses the model's adaptability to Zero-Day attacks, ensuring continuous improvement and effectiveness. This metric helps in fine-tuning the model's detection capabilities by providing feedback on its ability to adjust to new and unknown attack patterns.

In summary, the project's approach to Zero-Day DoS attack detection is characterized by its use of diverse data sources, adaptive and transfer learning mechanisms, attention to salient features through attention mechanisms, application of few-shot learning for generalization from limited data, continuous online learning for real-time adaptability, and innovative evaluation metrics for assessing adaptability. These strategies collectively enable the model to detect the unique and unpredictable characteristics of Zero-Day DoS attacks.


\section{State-of-the-Art}

In the domain of cybersecurity, particularly in the detection and mitigation of Distributed Denial of Service (DDoS) attacks, the state-of-the-art has evolved significantly to address the increasing complexity and frequency of these threats. Recent advancements have focused on leveraging machine learning (ML) and deep learning (DL) techniques to improve detection accuracy and response times. These approaches utilize extensive datasets to train models capable of identifying patterns indicative of DDoS activities, distinguishing them from legitimate network traffic. Deep learning, with its ability to learn complex patterns from data, has shown particular promise in this area. Models such as Convolutional Neural Networks (CNNs), Recurrent Neural Networks (RNNs), and variations like Long Short-Term Memory (LSTM) networks have been applied to parse and analyze network traffic, offering improved precision in identifying DDoS attacks over traditional signature-based and anomaly-based detection systems.

However, the emergence of Zero-Day DDoS attacks, which exploit previously unknown vulnerabilities, presents a significant challenge to these advanced detection methodologies. Zero-Day attacks elude conventional detection mechanisms that rely on known attack signatures or historical patterns. In response, researchers have begun to explore adaptive learning models and transfer learning techniques to enhance the detection framework's responsiveness to new and evolving threats. Adaptive models are designed to continuously learn and adjust to new data, enabling them to identify anomalies that could indicate a Zero-Day attack. Transfer learning allows these models to apply knowledge gained from detecting known attacks to identify new, related threats, thereby reducing the need for extensive retraining with new data. This shift towards models that can dynamically adapt to changing attack patterns represents a critical advancement in the field, setting the foundation for more resilient cybersecurity defenses against the ever-evolving landscape of DDoS threats.

The project under discussion advances the state-of-the-art by integrating these cutting-edge techniques into a comprehensive detection framework. By employing multi-modality data analysis, adaptive learning, and transfer learning within a deep learning architecture, it offers a novel approach to the detection of Zero-Day DDoS attacks. The use of multi-modality data enriches the model's training dataset, providing a more nuanced view of network behavior that can reveal subtle indicators of an attack. The adaptive learning component ensures that the model remains effective as attack strategies evolve, while transfer learning leverages existing knowledge to enhance detection capabilities with minimal additional training. This holistic approach, supported by ongoing advancements in machine learning and deep learning, represents a significant leap forward in the development of effective, adaptive cybersecurity measures capable of confronting the challenges posed by Zero-Day DDoS attacks.






\section{Related Work}
%\textcolor{red}{
%Michau et al. \cite{michau2021unsupervised} presented an advancement in anomaly detection through the development of an unsupervised transfer learning approach, specifically tailored for the transfer of complementary operating conditions. Their work showcases how this methodology can effectively identify anomalies by leveraging data from different but related operating environments, enhancing detection capabilities without the need for labeled data.
%
%Soltani et al. \cite{soltani2023adaptable} introduced an innovative deep learning-based Intrusion Detection System (IDS) that is adaptable to zero-day attacks. Their work demonstrates how the proposed IDS can dynamically adjust to newly emerging threats, ensuring robust protection against attacks that have not been previously identified or cataloged. This approach significantly enhances the security posture against unforeseen vulnerabilities and threats.
%
%Sarhan et al. \cite{sarhan2023zero} explored the application of zero-shot machine learning techniques for the detection of zero-day attacks. Their research outlines a novel approach that enables the identification of previously unknown cyber threats without direct prior knowledge or examples. This method promises to significantly improve the capability of security systems to preemptively recognize and mitigate emerging cyber attacks, addressing a critical challenge in cybersecurity.
%
%Jin et al. \cite{jin2023federated} introduced a Federated Incremental Learning-based Intrusion Detection System (IDS) that evolves to detect zero-day attacks. This approach combines the strengths of federated learning and incremental learning to create a system capable of adapting to new and unknown threats as they emerge. By leveraging data from distributed sources without compromising privacy, this system offers a scalable and effective solution for safeguarding against the ever-evolving landscape of cyber threats, specifically targeting the challenge of zero-day attacks.
%
%Wu et al. \cite{wu2024active} presented a novel active learning framework that incorporates Deep Q-Network (DQN) for the detection of zero-day attacks. This framework is designed to actively learn and adapt to new and previously unseen cyber threats, using a reinforcement learning approach to continuously improve its detection capabilities. By effectively identifying zero-day attacks, which are notoriously difficult to detect due to the lack of prior knowledge, this work offers a promising solution to enhance the security measures against sophisticated cyber threats in real-time.
%
%Verma et al. \cite{verma2023zero} introduced "Zero-Day Guardian," a dual-model federated learning framework specifically designed to counteract zero-day attacks in 5G-enabled Industrial Internet of Things (IIoT) environments. This framework employs two models within a federated learning context to enhance the detection and handling of zero-day attacks, which are particularly challenging due to their novel nature. By focusing on 5G-enabled IIoT, the research addresses the growing need for advanced security measures in increasingly connected and technologically sophisticated industrial systems.
%
%Li et al. \cite{li2023learning} explored a meta-learning approach tailored for unsupervised zero-day web attack detection across various web domains, despite the challenge of limited and heterogeneous training data. This study demonstrates how meta-learning can effectively leverage sparse and diverse data sources to enhance the detection capabilities for new and unknown web-based threats. By focusing on cross-domain applicability, the research significantly advances the field of cybersecurity, offering a promising strategy for identifying zero-day attacks in the dynamic and varied landscape of web domains.
%
%Debicha et al. \cite{debicha2023tad} introduced "TAD," a framework that applies transfer learning to enhance the detection of multi-adversarial evasion attacks targeting network intrusion detection systems. This approach addresses the challenge of adapting detection mechanisms to evolving threats by leveraging transfer learning, enabling the system to recognize and mitigate attacks that attempt to evade detection. By focusing on the dynamic and adversarial nature of cybersecurity threats, the TAD framework represents a significant step forward in developing more resilient and adaptable security measures for protecting network infrastructures.}


\section{Clarifications}
The Dual-Space Prototypical Network, as detailed in the proposal, is a novel deep learning framework optimized for detecting Distributed Denial of Service (DDoS) attacks, moving beyond traditional record-based methods. It utilizes a dual-space loss function to enhance the model's adaptability and sensitivity to both known and unseen DDoS attack vectors. This approach leverages the strengths of geometric and angular similarity measures to provide a more sophisticated understanding of class similarities, significantly improving performance across various attack scenarios even with small training sets.


The proposed novel deep learning framework, the Dual-Space Prototypical Network, is designed for detecting DDoS attacks by integrating an improved Prototypical Network that leverages a novel Dual-Space Loss. This loss function combines both Euclidean and cosine distance measures, enhancing the model's ability to recognize and adapt to new, unseen attacks even with limited training samples. Prototypical Networks, known for excelling in few-shot learning environments, learn to represent each class with a prototype, particularly effective when data is scarce. The training involves episodic scenarios, each simulating a few-shot learning challenge, to cultivate a resilient and adaptable model. The Dual-Space Loss aims to capture both the geometric proximity between embeddings and prototypes and their directional alignment, offering a more sophisticated understanding of class similarities. This approach significantly improves performance across various attack scenarios, even with small training sets, by exploiting the complementary strengths of geometric and angular similarity measures.


To improve the model's adaptability and sensitivity in terms of recognizing both known and unknown DDoS attack vectors, the proposal employs a dual-space loss function within the Dual-Space Prototypical Network. This loss function integrates both Euclidean distance (geometric distance) and cosine similarity (angular distance), enabling the model to evaluate the similarity between data points more holistically. This means the model can consider not only the magnitude of feature differences but also their directional alignment within the latent space. By leveraging this dual approach, the model gains a nuanced understanding of the data, which enhances its ability to adapt to new, unidentified attack patterns while maintaining high accuracy in recognizing established threats. This strategy allows for a more comprehensive representation learning, improving the model's effectiveness in a dynamic cybersecurity environment where adaptability and sensitivity to evolving threats are crucial.

The proposal justifies its claims of the framework's superior adaptability and learning efficiency through extensive evaluation across various training environments, including offline training, simulated online training, and prototypical network scenarios. This comprehensive evaluation demonstrates the model's robust performance under conditions of both data abundance and scarcity. Specifically, the Multilayer Perceptron (MLP) with Attention model trained in an online learning environment showcases high accuracy and an impressive F1-score, signifying its effectiveness in adapting to new data patterns—a critical requirement in cybersecurity. This demonstrates the model's adaptability to dynamic threat landscapes and establishes a new benchmark for adaptive cybersecurity defense strategies.

The "novel metric" introduced in the proposal is encapsulated by the dual-space loss function, symbolized as \(L_{D-space}\), crafted to quantify both geometric proximity and directional alignment amidst embeddings and prototypes. This metric is pivotal for nuanced class similarity discernment in few-shot learning scenarios, paramount in cybersecurity domains where novel attack instances are minimally available. The dual-space loss amalgamates normalized Euclidean distance (\(DE\)) and cosine distance (\(DC\)), facilitating a comprehensive similarity assessment between data points by considering both their magnitude differences and directional orientation within the latent space. Such an approach is adept at discerning intricate behavioral patterns emblematic of advanced DDoS assaults, thereby significantly elevating model performance across diverse attack situations, even with constrained training datasets. The metric's efficacy is corroborated through experimental evaluations, showcasing pronounced improvements over conventional methodologies and underscoring the strategy's enhanced capability in navigating the complex landscape of cybersecurity challenges.


\section{Contributions}


To address the concern from a technical contribution perspective, the proposal's focus shifts towards the specific innovations and advancements our research introduces in the detection and mitigation of DDoS attacks. Recognizing the limitations of traditional defense mechanisms that rely heavily on historical data, our work proposes a deep learning framework designed for adaptive, real-time detection and mitigation of both known and novel DDoS threats. This framework represents a significant leap forward in cybersecurity defenses, offering a comprehensive solution to a rapidly evolving challenge.

The cornerstone of our technical contribution lies in the development of an Adaptive Multi-Modality Deep Learning model that integrates several cutting-edge technologies. Firstly, we utilize a combination of Convolutional Neural Networks (CNNs) and Recurrent Neural Networks (RNNs) to process and analyze data streams in real-time. This combination allows for the extraction of temporal and spatial features within network traffic, enhancing the model's ability to distinguish between legitimate traffic and potential DDoS attack patterns.

Furthermore, we introduce a novel anomaly detection algorithm that leverages autoencoder networks. Unlike traditional threshold-based systems, this algorithm adapts dynamically to changing network behaviors, significantly reducing false positives while improving the detection of sophisticated, low-volume DDoS attacks that often go unnoticed.

Another significant contribution is the implementation of transfer learning techniques. By pre-training our model on diverse datasets from various network environments, it gains a broader understanding of potential attack vectors, improving its adaptability and effectiveness in unfamiliar settings. This approach addresses one of the critical challenges in DDoS defense: the ability to maintain high detection accuracy in the face of new or evolving attack methodologies.

Lastly, we emphasize the importance of ongoing learning and adaptation. Our framework incorporates a feedback loop that allows the system to learn from its successes and failures, continuously updating its detection algorithms based on new attack patterns and strategies identified in the wild. This feature ensures that the defense mechanism remains effective over time, even as attackers evolve their tactics.

In summary, our proposal's technical contributions provide a robust, adaptable, and highly effective solution to the challenge of DDoS attacks. By leveraging advanced deep learning techniques and a commitment to continuous improvement, we aim to significantly enhance the cybersecurity landscape's resilience against these pervasive threats.

\section{Comments}
\begin{itemize}
    \item deadline was extended to March 15.
    \item little disconnection still persists between introduction and actual model and evaluation
    \item compare with the most relevant paper (shared by Dr. Xin Ref. 19)
\end{itemize}
